Verifying Controllers with Convolutional Neural Network-based Perception: A Case for Intelligible, Safe, and Precise Abstractions

Convolutional Neural Networks (CNN) for object detection, lane detection, and segmentation now sit at the head of most autonomy pipelines, and yet, their safety analysis remains an important challenge. Formal analysis of perception models is fundamentally difficult because their correctness is hard if not impossible to specify. We present a technique for inferring intelligible and safe abstractions for perception models from system-level safety requirements, data, and program analysis of the modules that are downstream from perception. The technique can help tradeoff safety, size, and precision, in creating abstractions and the subsequent verification. We apply the method to two significant case studies based on high-fidelity simulations (a) a vision-based lane keeping controller for an autonomous vehicle and (b) a controller for an agricultural robot. We show how the generated abstractions can be composed with the downstream modules and then the resulting abstract system can be verified using program analysis tools like CBMC. Detailed evaluations of the impacts of size, safety requirements, and the environmental parameters (e.g., lighting, road surface, plant type) on the precision of the generated abstractions suggest that the approach can help guide the search for corner cases and safe operating envelops.

==> appx-nondet-sys.tex <==
\section{Generalized Definition }\label{appx:nondet-sys}

\chiao{TODO: Generalize definition to handle disturbance in dynamics with nondeterminism}

==> appx-tolerable.tex <==
\section{Proof for Tolerable Region}\label{appx:prove-tolerable}

==> sec-contract.tex <==
\section{Assume-Guarantee Contract}\label{sec:contract}

\newcommand{\Post}{\ensuremath{Post}\xspace}
\newcommand{\Spec}{\ensuremath{Spec}\xspace}
\newcommand{\err}{\ensuremath{\varepsilon_{env}}\xspace}

\newcommand{\Cert}{\ensuremath{\psi_\mathit{Cert}}\xspace}
\newcommand{\AppSum}{\ensuremath{\psi_\mathit{Apply}}\xspace}
\newcommand{\PCovX}{\ensuremath{\psi_\mathit{Init}}\xspace}
\newcommand{\PCovQ}{\ensuremath{\psi_\mathit{Seq}}\xspace}
\newcommand{\SatQ}{\ensuremath{\psi_\mathit{Sat}}\xspace}

Given $\Post: X \mapsto X$, a sequence of domains $X_0, \dots, X_n$ where $X_0 = X_n = X$, a collection of functions $f_i: X_{i-1} \mapsto X_i$ such that $\Post(x) = f_n \circ \cdots \circ f_1(x)$.
Without loss of generality, we use at most $m$ pairs $\langle P_{i,1}, Q_{i,1} \rangle \dotsc \langle P_{i,m}, Q_{i,m} \rangle$ of assume-guarantee contracts for each function $f_i$ where $P_{i,j} \subseteq X_{i-1}$ and $Q_{i,j} \subseteq X_{i}$.

Certify assume-guarantee contracts for each component $f_i$:
\begin{equation*}\label{eq:certify}
    \Cert \triangleq
    \bigwedge_{i=1}^n\bigwedge_{j=1}^m \forall x_{i-1}\in X_{i-1}, x_i\in X_i.
    \left(
        x_{i-1} \in P_{i,j} \land f_i(x_{i-1}) = x_i \implies x_i \in Q_{i,j}
    \right)
\end{equation*}

\Cert can be falsified with simulation when $f_i$ is only available as a black-box executable model.

\subsection{Proving Input-Output Specification using Assuming-Guarantee contracts}

Given input-output specification $\Spec(x_0, x_n)$, we want to prove
\begin{equation}\label{eq:exact-proof}
    \forall x_0\in X, x_n\in X, \Post(x_0) = x_n \implies \Spec(x_0, x_n)
\end{equation}

If certified assume-guarantee contracts are provided, we can weaken the premise of \eqref{eq:exact-proof} and derive:
\begin{equation}\label{eq:approx-proof}
\AppSum \land \PCovX \land \bigwedge_{i=1}^{n-1} \PCovQ^i \land \SatQ
\end{equation}

Apply assume-guarantee contract
\begin{equation*}
    \AppSum \triangleq
    \forall x_0\in X_0, x_1\in X_1, \dots, x_n\in X_n. \left(
        \left(
            \bigwedge_{i=1}^n\bigwedge_{j=1}^m x_{i-1} \in P_{i,j} \implies x_i \in Q_{i,j}
        \right) \implies \Spec(x_0, x_n)
    \right)
\end{equation*}

Covering Initial domain: $X_0 \subseteq \bigcup_{j=1}^m P_{1,j}$
\begin{equation*}
    \PCovX \triangleq
    \forall x_0 \in X_0. \left( \bigvee_{j=1}^m x_0 \in P_{1, j} \right)
\end{equation*}

Constraints for sequential composition:
$(\bigcup_{j=1}^m  Q_{i,j}) \subseteq (\bigcup_{j=1}^m P_{i+1,j})$ for all $i$,
or equivalently,
\begin{equation*}\label{eq:seq-compose}
    \PCovQ^i \triangleq  \forall x_i\in X_i.
    \left(
        \left(\bigvee_{j=1}^m x_i \in Q_{i,j}\right)
        \implies \left(\bigvee_{j=1}^m x_i \in P_{i+1,j}\right)
    \right)
\end{equation*}

Ensure contracts are satisfiable:
\begin{equation*}
    \SatQ \triangleq
    \bigwedge_{i=1}^n\bigwedge_{j=1}^m (P_{i,j} \neq \emptyset \implies Q_{i,j} \neq \emptyset)
\end{equation*}


\subsection{Relation with Parametric Assume-Guarantee Contracts}
Our theorem becomes a special case of parametric assume-guarantee contracts proposed in~\cite{kim_small_2017}
if we strengthen the constraint \PCovQ to be,
\[
\PCovQ \triangleq
\bigwedge_{i=1}^{n-1} \bigwedge_{j=1}^m \forall x_i\in X_i. 
    \left(
        x_i \in Q_{i,j} \implies x_i \in P_{i+1,j}
    \right)
\]
where we select a parameter $j$ from the discrete parameter space $\{1,\dotsc, m\}$, and the parameter map $\lambda_i$ is simply an identity map for all functions $f_i$.


\section{Presume-Achieve Contract for Must analysis}

\newcommand{\uP}{\ensuremath{P^-}\xspace}
\newcommand{\uQ}{\ensuremath{Q^-}\xspace}

A presume-achieve contract $\langle \uP_i, \uQ_i \rangle$ for the function $f_i$ has to ensure that, for every output $y$ in $\uQ_i,$ there exists an input $x$ in $\uP_i$ which produces $y=f_i(x)$.
Formally,
\[
\psi^-_\mathit{Cert} \triangleq \forall y \in \uQ_i. \exists x \in \uP_i. (y = f_i(x))
\]

Sequential composition, $\uP_{i+1} \subseteq \uQ_{i}$
\[
\psi^-_\mathit{Seq} \triangleq \forall x_i \in X_i. (x_i \in \uP_{i+1} \implies x_i \in \uQ_{i})
\]
